Nesterov's method with decreasing learning rate leads to accelerated stochastic gradient descent

We present a coupled system of ODEs which, when discretized with a constant time step/learning rate, recovers Nesterov's accelerated gradient descent algorithm. The same ODEs, when discretized with a decreasing learning rate, leads to novel stochastic gradient descent (SGD) algorithms, one in the convex and a second in the strongly convex case. In the strongly convex case, we obtain an algorithm superficially similar to momentum SGD, but with additional terms. In the convex case, we obtain an algorithm with a novel order $k^{3/4}$ learning rate. We prove, extending the Lyapunov function approach from the full gradient case to the stochastic case, that the algorithms converge at the optimal rate for the last iterate of SGD, with rate constants which are better than previously available.

==> sections/Acc_LatexCommands.tex <==


\newtheorem{theorem}{Theorem}[section]
\newtheorem{principle}{Principle}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newcommand{\R}{\mathbb{R}}
\newcommand{\CCff}{{C_f}^{-1}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}



==> sections/Liap_GD.tex <==
%\newcommand{\minx}{x_*}
%\newcommand{\minf}{f^*}
%\newcommand{\minz}{z_*}
%\newcommand{\minp}{p_*}


 
\section{Abstract Liapunov Analysis: going from continuous to discrete time}
\blue{discussion, TODO}
Continuous time approach to first order convex optimization with application to GD, AGD, SGD and accelerated SGD. Huge literature on the nesterov and continuous time and ODEs
* Goal of the literature not completely well-defined.  Appears to be a consensus that cts time analysis can offer a framework for optimization.  May lead to more understandable proofs.
* However, the project of cts analysis to discrete is still not clearly defined.  Which liapunov functions.
* Already a literature in applied math on Liap (textbook stuart).   However, these methods mostly implicit.  Closest connection would be to Catalyst, or proximal gradient method.  Know these methods automatically are descent methods, and each step decreases Liapunov.  Nice theory, but pushes the full analysis one step away to solving the subproblem.  Can be effective if can treat the subproblem as a black box.
* Here: we make a definition of the continuous to discrete problem.  Make a discinction between the simpler exact discretiation case, and the perturbed case.  The former is simpler, and works for desecent methods.  The latter is somehwat more complex, because there is a larger search space, but works for acceleration. 
* Success of the framework: we can treat both the full gradient and the stochastic gradient case. 



\subsection{Definitions and framework}
Our goal here is to obtain rates for optimization algorithms using a continuous time perspective.  The idea put forward by many authors, notably [jordan]? is that the convergence proofs of accelerated algorithms do not give enough insight, and that building the connection with continuous time methods may bring the insight needed to more easily develop new algorithms. 


To explain the general idea, consider an abstract Ordinary Differential Equation (ODE), generated by the velocity field $g: \R^n \to \R^n$ which is  $L_g$-Lipschitz continuous. 
\begin{equation}\label{abstractODE}\tag{ODE}
	z'(t) = g(z(t))
\end{equation}
Then \eqref{abstractODE}  has unique solutions in all time for every  initial condition $z(0) = z_0 \in \R^n$. 

For a given learning rate (time step) $h \geq 0$, to the forward Euler discretization of  \eqref{abstractODE} corresponds to the sequence 
\begin{equation}\label{abstractFE}\tag{FE}
	z_{k+1} = z_k + h g(z_k)
\end{equation}
provided an initial value $z_0$.
The solution of \eqref{abstractFE} can be interpolated to be a function time by defining the time steps $t_k = hk$ and defining the function $z^h : [0,T) \to \R^n$ by  
\[
z^h(t_k) = z_k
\]
and using piecewise constant (or linear)  interpolation in between time steps \blue{Define interpolation more precisely, make consistent with quadrature} .  It is a standard result from numerical analysis of ODE  theory~\cite{iserles2009first} that functions $z^h$ converge to $z(t)$ with error of order $h$, provided $h \leq 1/L_g$. 
%

\begin{definition}
The function $E(z,t)$ is a Liapunov function for \eqref{abstractODE} if 
\begin{equation}\label{abstractLIAP}
	\frac{d}{dt} E(z(t),t) \leq 0.
\end{equation}
for every solution $z(t): [0,\infty) \to \R^n$ of \eqref{abstractODE}. 
%\blue{maybe define LIAPUNOV with gap and put in the that gape is $t |\nabla f|^2$ for the conts time} 
%
If, in addition, there is an $h_0 > 0$ so that 
\begin{equation}\label{discreteLIAP}
	E(z_{k+1},t_{k+1}) \leq E(z_k, t_k)
\end{equation}
for all solutions $z_k$ of \eqref{abstractFE} with  $0 < h \leq h_0$, then we call $E$
a Liapunov function for the sequence~\eqref{abstractFE}. 
\end{definition}

In fact, as we show below, for (non-accelerated) gradient descent, in both the convex and strongly convex case, the setup \eqref{discreteLIAP} holds: we can directly discretize the ODE and the Liapunov function.     In fact, in continuous time, we will show something stronger than \eqref{abstractLIAP}: there will be a gap in the inequality.  It is the gap in the inequality which can be exploited to obtain the inequality \eqref{discreteLIAP}. 







\begin{theorem}\label{Thm:ConvexLiapNoAcc}
Suppose $f(x)$ is convex and $L$-smooth. Define the gradient descent velocity field 
\begin{equation}
	\label{vel_GD}
		g(x(t)) = - \nabla f(x(t))
\end{equation}
and define
\begin{equation}\label{Liap_GD}
		E^c(x,t)  = t(f(x)-\minf) +\frac 1 2 |x-\minx|^2
\end{equation}
Then $E^c$ is a continuous Liapunov function (with gap $t|\nabla f(x)|^2$) and a Liapunov function for the sequence generated by \eqref{abstractFE} 
applied to \eqref{abstractODE} \eqref{vel_GD}  with  $h_0 = 1/L$.   
Suppose, in addition, that $f(x)$ is $\mu$-strongly convex.  Then 
\begin{equation}\label{E_defn}
E^{sc}(x,t) = \frac 1 2 \exp(\mu t ) |x-\minx|^2
\end{equation}
is also Liapunov function for the sequence generated by \eqref{abstractFE} 
applied to \eqref{abstractODE} \eqref{vel_GD}  with  $h_0 = 1/L$.   
\end{theorem}

In the convex case, the Liapunov  function, $E^c$ gives the $1/t$ rate which corresponds to $hk = t_k$ with the optimal rate given by $h = h_0 = 1/L$. 

[[ See \S\ref{Sec:ProofNoAcc}  for the proof ]]


\subsection{Liapunov analysis for accelerated algorithms}
However, the situation is not quite so simple in the accelerated case.  First note that there is a gap between the discrete and continuous setting: more than one ODE can be consistent with a discrete algorithm.   This means, in principle, that there may be whole parameterized families of ODEs which satisfy the condition \eqref{abstractLIAP} and which can be discretized to obtain the algorithm.   In the accelerated case, we need to use such a parameterized family. 

For the accelerated case, it may be too restrictive to require that the Forward Euler discretization of the ODE satisfies the same Liapunov function.  However, we can consider a perturbed ODE system.  (And we may need to consider a perturbed Liapunov function)

Consider the parameterized velocity field $g(x;t,h)$ which is  $L_g$-Lipschitz continuous, uniformly in $h$.   In continuous time, set $h = 0$, and consider
\begin{equation}\label{PabstractODE}\tag{ODE-h}
	z'(t) = g(z(t),t;0)
\end{equation}
However, for a given learning rate (time step) $h \geq 0$, we allow a perturbation which depends on $h$, and instead consider the algorithm 
\begin{equation}\label{PabstractFE}\tag{FE-h}
	z_{k+1} = z_k + h g(z_k,t; h)
\end{equation}
provided an initial value $z_0$.

\begin{definition}
The (continuous) function $E(z,t;h)$ is a Liapunov function for \eqref{PabstractODE} if 
\begin{equation}\label{abstractLIAP}
	\frac{d}{dt} E(z(t),t;0) \leq 0.
\end{equation}
for every solution $z(t): [0,\infty) \to \R^n$ of \eqref{PabstractODE}. 
If, in addition, there is an $h_0 > 0$ so that 
\begin{equation}\label{discreteLIAP}
	E(z_{k+1},t_{k+1};h) \leq E(z_k, t_k;h)
\end{equation}
for all solutions $z_k$ of \eqref{abstractFE} with  $0 < h \leq h_0$, then we call $E$
a Liapunov function for the sequence~\eqref{abstractFE}. 
\end{definition}



\subsection{just convert this section to give the proof in the Strongly convex case}
 

Let $E(z)$ be a $\mu_E-$strongly convex function $E(z)$ with $L_E$ smoothness parameter. Write $\minz$ for the  minimizer of $E$. 

Consider the ode
\begin{equation}\label{ODEz}
		z'(t) = v(t,z(t))
\end{equation}
The forward Euler method is given by 
\begin{align}
	\label{FE}\tag{FE}
	\frac{z_{k+1}-z_k}{h} &= v(t_k,z_k) 
%	\\
%	\label{BE}\tag{BE}
%	\frac{z_{k+1}-z_k}{h} &= v(t_{k+1},z_{k+1}) 
\end{align}

\begin{definition}
 We say $E$ is a rate-generating Liapunov function for \eqref{ODEz} if there are constants $r_E >0, a_E \geq 0$ such that 
\begin{equation}\label{Liap_Cond}
 \nabla E(z) \cdot v(t,z) \leq - r_E E(z(t)) - a_E |v(t,z(t))|^2
\end{equation}
\end{definition}

\begin{lemma}
Let $E$ be a rate generating Liapunov function for \eqref{ODEz}. 
Then 
\[
E(z(t)) \leq E(z(0)) \exp(-r_Et)
\]
\end{lemma}
\begin{proof}
\[
		\frac{d}{dt}E(z(t))  = \nabla E \cdot v \leq - r_E E(z(t)) - a_E |v(t,z(t))|^2
\]
by assumption \eqref{Liap_Cond}. Gronwall's inequality gives the result.
\end{proof}

\begin{lemma}\label{lem:FEconvergenceLIAP}
	Let $z_k$ be the solution of the forward Euler method \eqref{FE} for \eqref{ODEz} with time step $h > 0$.  
	Let $E$ be a rate generating Liapunov function for \eqref{ODEz} with constant $a_E > 0$ so that \eqref{Liap_Cond} holds.  Suppose
	\begin{equation}
		\label{CFL}\tag{CFL}
		h \leq \frac{2 a_E}{L_E}
	\end{equation}
Then 
\begin{equation}
	E(z_{k+1})  \leq (1 - h r_E) E(z_k)
\end{equation}
In particular, choosing equality in \eqref{CFL} we have 
\begin{equation}\label{FE_rate}
	E(z_{k})  \leq \left(1 - \frac {2 a_E r_E }{L_E}\right)^k E(z_0)
\end{equation}
\end{lemma}

\begin{proof}
Estimate $E_{k+1}- E_k$ using 1-convexity to get
\begin{align}
E(z_{k+1})- E(z_{k}) &\leq \nabla E(z_{k})(z_{k+1}- z_{k}) + \frac {L_E} 2 |z_{k+1}- z_{k}|^2\\
& \leq 	- hr_E E_{k} - ha_E |v_{k+1}|^2 + \frac {h^2 L_E} 2 |v_{k+1}|^2 && \text{by \eqref{FE} and \eqref{Liap_Cond}}
\end{align}
So apply \eqref{CFL} to get
\[
E(z_{k+1})- E(z_{k}) \leq - hr_E E_{k} = - \frac {2 a_E r_E }{L_E}E_{k}
\]
which gives \eqref{FE_rate}.
\end{proof}


\section{Accelerated convex case}
Define the perturbed ODE by setting $z = (x,v)$ and $g(x,v,t,h)$ as follows.  Then define
\begin{equation}\label{gh_defn}
	\begin{aligned}
		g^1(x,v,t;h) &= \frac{2}{t}(v-x) -\frac{1}{\sqrt{L}}\nabla f(y^h),\\
		g^2(x,v,t,h) &= - \frac{t}{2}  \nabla f(y^h)
\end{aligned}
\end{equation}
where we define the auxiliary variable
\begin{equation}
	\label{yh_defn}
	y^h = y(x,v,t;h) =   x + \frac{2h}{t}(v-x)
\end{equation} 


Let $h>0$ be a given small time step/learning rate and let $t_k= h(k+2)$.
 The forward Euler method for $g$ is given by
\begin{equation}
\label{FEg}\tag{FE-C}
\left \{
\begin{aligned}
	x_{k+1} - x_k &= \frac{2h}{t_k} (v_k - x_k) - \frac{h}{\sqrt{L}}\nabla f(y_k),\\
v_{k+1} - v_k &= -\frac{h  t_k}{2}\nabla f(y_k)		
\end{aligned}
\right .
\end{equation}
where 
\begin{equation}
\label{yk_defn}
y_k =   \frac{k x_k  + 2 v_k}{k+2}.
\end{equation}




\blue{ TODO move the k, k+1, k+2, and can we shuffle the definitions to get this to fit? } 

\begin{definition}
Define the continuous time parameterized Liapunov function
\begin{equation}\label{LiapCTS}
 E(t,x,v,h ):= (t-h)^2( f(x) - f^* ) +2|v - x^* |^2
\end{equation}	
Define the discrete time Liapunov function $E_k$ by 
\begin{equation}
	\label{Ek_defn}
%	E_k = E(t_{k-1}, x_k, v_k) %= t_{k-1}^2 (f(x_k) - f^*) + 2|v_k-x^*|^2,
	E_k =  E(t,x,v;h ) = E(t_{k-1}, x_k, v_k)  \blue{~ makes this fit} 
\end{equation}
%where $E$ is given by \eqref{LiapCTS}. 
\end{definition}


\begin{theorem}\label{Thm:ConvexLiapNoAcc}
Suppose $f(x)$ is convex and $L$-smooth. 
Define the velocity field by \eqref{gh_defn} and let $E$ be given by \eqref{LiapCTS}.
Then $E$ is a  continuous Liapunov function (with gap $t^2|\nabla f(x)|^2$) and a discrete Liapunov function for the sequence generated by \eqref{FEg} 
\begin{equation}\label{h_cond}
	h_0 = \frac{1}{ \sqrt{L}}
\end{equation}
\end{theorem}

\blue{TODO merge this one to previous one } 

Can say : we show we get Nesterov, so part of the proof is done. 
The main step is the discretization.  Also include the proof in continous time.
 
 Since   \eqref{FE} is equivalent to Nesterov's method, the rate is known. The proof of the rate using a Liapunov function can be found in \cite{beck2009fast}. A proof which shows that we can use the constant time step can be found in~ \cite{beck2017first}. The discrete Liapunov function 
 \eqref{Ek_defn} was used in \cite{su2014differential,Attouch2016faster} to prove a rate.  

\begin{remark}
	Note, compared to the ODE from Su-Boyd, the cts time ODE has the gap, which would not be there if the extra terms was missing.  So maybe this is a better ODE?  In particular, if $\tilde z$ solution of su-boyd and $z$ solution of ourse, then we can prove  faster convergnce due to the gap.   
\end{remark} 
 
\begin{proposition}
\label{prop: rate convex continuous p=2}
\label{prop: discrete convex p=2}
Let $f$ be a convex and $L$-smooth function. 
Let $(x(t),v(t))$ be a solution to \eqref{NODE}, then 
\[
 \frac{d E(t,x(t),v(t))}{dt} \leq -\frac{ t^2}{\sqrt{L}}  |\nabla f(x) |^2 .
 \]
 where  $E(t,x,v)$ in given by \eqref{LiapCTS}. In particular, for all $t>0$,
\[
f(x(t)) - f^* \leq \frac{2}{ t^2} |v_0 -x^* |^2.
\]
Furthermore, let $x_k,v_k$ be given by \eqref{FEg}.   Then for all $k\geq 0$, 
\[
E_{k+1} \leq E_k -h^2(f(x_k) - f^*) + \left( h - \frac{1}{\sqrt{L}} \right) t_k^2h |\nabla f(y_k) |^2.
\]
In particular, if 
\begin{equation}\label{h_cond}
	h \leq \frac{1}{ \sqrt{L}}
\end{equation}
then $E_k$ is decreasing. When equality holds in \eqref{h_cond},
\[
f(x_k) - f^* \leq \frac{ 2 }{(k+1)^2}\left( (f(x_0) - f^*) +  |v_0-x^*|^2\right).
\]
\end{proposition} 

 
 The proof of the continuous time part is short, and so we include it here. 
\begin{proof}[Proof of Prof~\ref{prop: rate convex continuous p=2}]
By definition of $E$, we have
%
\begin{eqnarray*}
\frac{d E}{dt}  
&\leq   & 2t(f(x) - f^*) + t^2 \langle \nabla f(x) , \dot{x} \rangle\\
&& + 4\langle v - x^* , \dot{v} \rangle \\
&\leq & 2t( f(x) - f^*)  +2 t  \langle \nabla f(x) , v - x \rangle - \frac{ t^2}{\sqrt{L}}|\nabla f(x) |^2\\
&&  -2t  \langle v - x^*, \nabla f(x) \rangle\\
& \leq & 2t ( f(x) - f^* - \langle x - x^* , \nabla f(x) \rangle )  - \frac{ t^2}{\sqrt{L}} |\nabla f(x) |^2. 
\end{eqnarray*}
% 
The proof is concluded by convexity, 
\[ f(x) - f^* - \langle x - x^* , \nabla f(x) \rangle \leq 0. \qedhere
\]
%
\end{proof}




\subsection{Stochastic Abstract Liapunov}

 Next, in the stochastic case, we can consider the perturbed ODE
\begin{equation}
	z'(t) = g(z) + e
\end{equation}
and an augmented Liapunov function
\begin{equation}
	E(z) + I(z(\cdot))
\end{equation}
where $I$ is an integral function of the curve $z(s), 0\leq s \leq t$. 
Similarly, using the same argument, the perturbed augmented Liapunov function 
\begin{equation}
	E(z_k) + I(z(\cdot))
\end{equation}
where $I$ is the same integral function evaluated on the piece-wise constant curve $z(h k), k = 0, \dots, T$
\begin{equation}
	z_{k+1}-z_k = h g(z_k;h) + e_k
\end{equation}
discretization corresponds to a  \dots 












==> sections/Liap_SGD.tex <==






\section{Stochastic Gradient Descent (not accelerated)}
\label{Appendix: SGD}


\subsection{SGD no Acc, Convex case: continuous and discrete time}
We begin with the assumption on the error term in the stochastic gradient.
Assume
\begin{equation}
	\label{ass:SGD}
	 e\, : \, [0, +\infty) \rightarrow {\R}^d \text{ is an integrable function}
\end{equation}
a sufficient condition which implies \eqref{ass:SGD} is that
\begin{equation}
	\label{ass:SGDw}
	|e(t)| \leq \frac 1 {t^{1+\alpha}}
\end{equation}
for some constant $\alpha > 0$. 

Consider the gradient descent 
%
\begin{eqnarray}
\label{eq: SGD convex}
\dot{x} = - ( \nabla f(x) +e(t)).
\end{eqnarray}
%
Then define the Lyapunov function, $\tilde{E}$, by
%
$$  \tilde{E}(t,x) = E(t,x) + I(t),$$
%
where,
%
$$ E(t,x) = t(f(x) -f^*) +\frac{1}{2}|x-x^*|^2,$$
%
and,
%
$$ I(t) = \int_0^t \langle x(s)- x^* +s\nabla f(x(s)) , e(s) \rangle \,ds.$$

Then the following result holds.

\begin{proposition}
\label{prop: SGD convex continuous}
Let $x$ be a solution of \eqref{eq: SGD convex} with initial condition $x_0$. Then,
%
$$\frac{d \tilde{E}(t,x)}{dt} \leq - t | \nabla f(x)|^2.$$
%
In addition, if $f$ is $L$-smooth, then 
\[
\sup_{s \geq 0} |x(s) -x^*| <+\infty
\] and
\[
\sup_{s \geq 0} s|\nabla f(x(s))| <+\infty
\]
and thus 
\blue{ maybe put a constant in here } $\|I \|_\infty$ 
\[
 f(x(t)) -f^* \leq \frac{1}{t}\left( f(x_0) -f^* +\frac{1}{2}|x_0 - x^*|^2 + \sup_{s \geq 0} |x(s) -x^* + s\nabla f(x(s))| \| e \|_{L^1(0,+\infty)} \right).
 \]
\end{proposition}


\begin{proof}
For all $t>0$, we have
\begin{itemize}
\item $\frac{d E(t,x)}{dt} = (f(x) -f^* -\langle \nabla f(x), x -x^* \rangle) -t|\nabla f(x) | - \langle x -x^* + t\nabla f(x) , e\rangle$,

\item $\frac{d I(t)}{dt} =  \langle x -x^* + t\nabla f(x) , e\rangle$.
\end{itemize}

Then, since $f$ is convex, we obtain the first result. We deduce that $\tilde{E}$ is decreasing. Arguing as \cite{attouch2016fast} along with the co-coercivity inequality, we prove that $\sup_{s \geq 0} |x(s) -x^*| <+\infty$, $\sup_{s \geq 0} s|\nabla f(x(s))| <+\infty$ which concludes the proof.
\end{proof}


The discretization of \eqref{eq: SGD convex} is 
%
\begin{eqnarray}
\label{eq: dicrete SGD convex}
x_{k+1} -x_k  = - h( \nabla f(x_k) +e_k),
\end{eqnarray}
%
where $e_k= e(hk)$. 


Define $\tilde{E}_k$ by
%
$$ \tilde{E}_k = E_k +I_k,$$
%
where, for $t_k:=hk$,
%
$$ E_k= t_k( f(x_k) -f^*) +\frac{1}{2}|x_k -x^* |^2,$$
%
and,
%
$$ I_k = h\sum_{i=0}^{k-1} \langle x_i - x^* -t_{i+1}( \nabla f(x_{i}) +e_{i}), e_{i} \rangle.$$ 

\begin{proposition}
Let $x_k$ be the sequence generated by \eqref{eq: dicrete SGD convex} with initial condition $x_0$. Assume that $h$ satisfies, for all $k\geq 0$,

%
\begin{equation}
	\label{ass: time step discrete SGD convex}
h \leq \frac{1}{L}.
\end{equation}

\begin{eqnarray}
\label{ass: time step discrete SGD convex}
h(Lt_{k+1} +1) -2 t_{k+1} \leq 0 \equiv h \leq \frac{1}{L}.
\end{eqnarray}
\blue{ move this down into proof? }
%
Then the $\tilde{E}_k$ is decreasing. In addition if $(e_k)_k$ and $(t_{k+1} |e_k|^2)_k$ are summable, $\sup_{i \geq 0} |x_i -x^*| <+\infty$, $\sup_{i \geq 0} |t_{i+1} \nabla f(x_i)| <+\infty$ and
%
$$ f(x_k) -f^* \leq \frac{1}{t_k}\left[\frac{1}{2}|x_0 -x^* |^2 + \sup_{i \geq 0} |x_i -x^*+t_{i+1}\nabla f(x_{i})| \sum_{i=0}^{+\infty} (|e_i| + t_{i+1}|e_i|^2)  \right].$$
\end{proposition}


\begin{proof}
By $L$-smoothness and convexity of $f$, we have
%
\begin{eqnarray*}
E_{k+1} - E_k & \leq & -h t_{k+1} \langle \nabla f(x_k), \nabla f(x_k) +e_k \rangle \\
& & +( Lt_{k+1} +1)\frac{h^2}{2}|\nabla f(x_k) +e_k |^2 \\
&& - \langle x_k -x^* , e_k \rangle\\
&& +h(f(x_k) -f^* - \langle \nabla f(x_k) , x_k -x^* \rangle)\\
& \leq & ( (Lt_{k+1} +1)h - 2t_{k+1})\frac{h}{2}|\nabla f(x_k) +e_k |^2 \\
&& - h\langle x_k -x^* , e_k \rangle + t_{k+1}h \langle \nabla f(x_k) +e_k , e_k \rangle.
\end{eqnarray*}
%
In addition,
%
$$ I_{k+1} -I_k =  h\langle x_k - x^* -t_{k+1}( \nabla f(x_{k}) +e_{k}), e_{k} \rangle,$$
%
therefore,
%
$$ \tilde{E}_{k+1} -\tilde{E}_k \leq ( (Lt_{k+1} +1)h - 2t_{k+1})\frac{h}{2}|\nabla f(x_k) +e_k |^2 \leq 0,$$
%
when $h$ satisfies \eqref{ass: time step discrete SGD convex}. We conclude the proof with the same argument as Proposition \ref{prop: SGD convex continuous}.  
\end{proof}






==> sections/N2N_Convex_AA.tex <==




\section{Accelerated method: convex case}
\label{section: accelerated convex}
In the remainder of the paper, we will extend the analysis developed in Section~\ref{section:application} to the accelerated gradient methods and, in this section, we consider the case of convex function.
%We study the perturbed case as in the full gradient descent case. However, we will see, in the perturbed case, that the definition of $I$ requires slight modifications. Indeed, the Lyapunov function and the gradient of $f$ are not evaluated at the same point. We will also consider the case where the time step is varying and the error has zero-mean and a constant variance. Section \ref{section: accelerated convex} considers the convex case while Section \ref{section: accelerated str convex} focuses on the strongly convex case. 
%
%
%In this section, we study system \eqref{NODE} as well as its discretization \eqref{FEg}. Then we extend the Lyapunov analysis to the perturbed case. We present also a convergence rate for the expectation of $f$ in the case of the time step varies, $h_k$, and the error has a constant variance. 
\subsection{ODE and derivation of Nesterov's method}

In the notation \eqref{g_affine}, \eqref{NODE} corresponds to the case $z=(x,y)$ and 
\begin{equation*}
%\label{eq: velocity field acc convex 1}
g(t,x,v,\nabla f(x))= \begin{pmatrix}
-\frac{2}{t} & \frac{2}{t}  \\
0 & 0
\end{pmatrix} 
z' 
+ \begin{pmatrix}
-\frac{1}{\sqrt{L}}   \\
-\frac{t}{2}
\end{pmatrix}\nabla f(x),
\end{equation*}




%Recently in \cite{shi2018understanding}, Shi, Du, Jordan and Su introduced a family of second order differential equations called high-resolution differential equation. This equation is derived from Nesterov's method using terms of order $\mathcal{O}(1)$ and $\mathcal{O}(h)$ instead of only terms of order $\mathcal{O}(1)$ to derive \eqref{ODE_Su}. In this context, \eqref{OurEqnCC} corresponds to the high-resolution equation with the parameter $\frac{1}{\sqrt{L}}$. In this case, in~\eqref{OurEqnCC} the coefficient of $\dot{x}$ is damped by the Hessian and then depends on $x$. In addition, the coefficient of $\nabla f(x)$ is perturbed by $\frac{1}{\sqrt{L}t}$ which goes to zero asymptotically. This equation corresponds at a first order perturbation $\mathcal{O} \left( h=\frac{1}{\sqrt{L}}\right)$ of \eqref{ODE_Su}.    The system \eqref{NODE} can be discretized to recover Nesterov's method using a explicit discretization with a constant time step $h=\frac{1}{\sqrt{L}}$, as demonstrated in Proposition~\ref{prop: discret Nest convex}.


% By a Lyapunov analysis, we recover the usual optimal rates, in both continuous and discrete cases, and, in addition, we obtain an extra gap in the dissipation of the Lyapunov function, Proposition \ref{Thm:ConvexLiapNoAcc}, which gives us an estimate on the decrease of $|\nabla f(x)|^2$, Corollary \ref{cor: decrease gradient}.  
%Moreover, another advantage of the first order system, is that it can be extended to non-smooth functions and to the perturbed case as we will see in Sections~\ref{section: accelerated convex}.  
%The extra term in system \eqref{NODE} will give a extra gap in the dissipation of the Lyapunov function as well as a better rate of convergence on the gradient, see Section \ref{section: accelerated convex}.	

Nesterov's method  for a convex, $L$-smooth function, $f$,  can be written as \cite[Section 2.2]{nesterov2013introductory}
\begin{equation}
	\label{sys: Nesterov convex}\tag{C-Nest}
\left \{
\begin{aligned}
	x_{k+1}  &= y_k - \frac 1 L \nabla f (y_k)\\
	y_{k+1} &=x_{k+1} + \frac{k}{k+3}(x_{k+1} -x_k)	
\end{aligned}
\right .
\end{equation}

%Note that to obtain Nesterov's method, the gradients are evaluated at $y_k$ which is a . 
\begin{definition}
Let $h_k>0$ be a decreasing sequence of small time step/learning rate and $t_k$ an increasing sequence of discrete time. The discretization of \eqref{NODE} corresponds to an explicit time discretization with gradients evaluated at $y_k$, the convex combination of $x_k$ and $v_k$, defined below, 
% = \left(1-\frac{2}{k+2}\right) x_k  + \frac{2}{k+2} v_k$ is given by
\begin{equation}
\label{FEg}\tag{FE-C}
\begin{cases}
	x_{k+1} - x_k = \frac{2h_k}{t_{k}} (v_k - x_k) - \frac{h_k}{\sqrt{L}}\nabla f(y_k),\\
    v_{k+1} - v_k = -\frac{h_k  t_{k}}{2}\nabla f(y_k),\\
	y_k =   \left(1-\frac{2h_k}{t_{k}}\right) x_k  + \frac{2h_k}{t_{k}} v_k.	
\end{cases}
\end{equation}	
\end{definition}

Then the following result holds.
\begin{proposition}
\label{prop: discret Nest convex}
The discretization of \eqref{NODE} given by \eqref{FEg} with $h_k=h = 1/\sqrt{L}$ and $t_k = h(k+2)$
is equivalent to the standard Nesterov's method \eqref{sys: Nesterov convex}. 
\end{proposition}





\subsection{Perturbed gradient: discrete time}
Replacing gradients with $\tilde{\nabla }f = \nabla f +e$, the discretization of \eqref{NODE}, \eqref{FEg}, with a time step $h_k$, becomes
\begin{equation}
\label{FE_Stoc}\tag{Per-FE-C}
\left \{
\begin{aligned}
x_{k+1} - x_k &= \frac{2h_k}{t_{k}}(v_k-x_k) - \frac{h_k}{\sqrt{L}} (\nabla f(y_k) +e_k),\\
v_{k+1} - v_k &=  -  h_k\frac{t_{k}}{2} (\nabla f(y_k) +e_k),
\end{aligned}
\right. 
\end{equation}
%
where $y_k$ is as in \eqref{FEg}, $t_k = \sum_{i=0}^k h_i$.\\

\begin{definition}
Define the continuous time parametrized Lyapunov function
\begin{equation}\label{LiapCTS}
 E^{ac,c}(t,x,v;\epsilon ):= (t-\epsilon)^2( f(x) - f^* ) +2|v - x^* |^2
\end{equation}	
Define the discrete time Lyapunov function $E_k^{c}$ by 
\begin{equation}
	\label{Ek_defn}
	E_k^{ac,c} =  E^{ac,c}(t_k,x_k,v_k ;h_k) =E^{ac,c}(t_{k-1},x_k,v_k ;0)  
\end{equation}
%where $E$ is given by \eqref{LiapCTS}. 
\end{definition}


It is well-known that $E^{ac,c}$ is Lyapunov function for \eqref{NODE}, see \cite{su2014differential}. But note, compared to Su-Boyd-Cand\'es' ODE \eqref{ODE_Su}, there is a gap in the dissipation of the Lyapunov function $E^{ac,c}$, which will not be there if the extra term, $-\frac{1}{\sqrt{L}}\nabla f(x)$, was missing, see Appendix \ref{appendix: acc convex lyap analysis continusous unperturbed}.  In particular, if $z$ and $\tilde z$ are solutions of \eqref{ODE_Su} and \eqref{NODE} respectively, then we can prove faster convergence due to the gap.

\begin{proposition}
\label{prop: different gaps convex acc perturbed}
Let $x_k,v_k,y_k$ be sequences generated by \eqref{FE_Stoc}-\eqref{FEg}. Then, for $h_k \leq  \frac{1}{\sqrt{L}}$,
\begin{equation}
\label{eq:main inequality E convex acc perturbed}
E_{k+1} ^{ac,c}- E_k^{ac,c} \leq  h_k\beta_k,
\end{equation}
where $\beta_k  :=  -t_{k} \langle 2(v_k -x^*) ,e_k - \frac{t_{k}}{\sqrt{L}} \nabla f(y_k) , e_k \rangle + 2h_k t_{k}^2 \left\langle \nabla f(y_k) +\frac{e_k}{2},e_k \right\rangle$.
\end{proposition}






\subsection{Convergence in expectation}
\label{subsection: variable time step acc convex}
Assume $e_k$ satisfies \eqref{ass: mean and varience error}. We deduce that $\mathbb{E}[\beta_k] = h_kt_k^2 \sigma^2$. Then, Proposition \ref{prop: different gaps convex acc perturbed} gives
\[
\mathbb{E}[E^{ac,c}_{k+1} ] - E^{ac,c}_{k} \leq h_k^2t_k^2 \sigma^2.
\]
In addition,
\[
\mathbb{E}[E^{ac,c}_{k} ]  \geq t_{k-1}^2 \mathbb{E}[f(x_{k})] -f^*.
\]
That corresponds to \eqref{ass: expectation E_k r_E=0 1} and \eqref{ass: expectation E_k r_E=0 2} with
\begin{equation}
\label{eq: values a_i and b_i acc Convex}
a_1=a_2 =0, \,  a_3 = 2, \, b_1=0 \text{ and }b_2 =1.
\end{equation} 

Then we can apply Proposition \ref{prop: decrease expectation E_k r_E=0} to obtain the following convergence results.

\begin{proposition}
\label{prop: decrease expectation E_k convex acc}
Assume $h_k := \frac{c}{k^{\alpha}} \leq \frac{1}{\sqrt{L}}$ and $t_k =\sum_{i=1}^k h_i$, then the following holds:
%\begin{eqnarray*}
%\mathbb{E}[f(x_k)] - f^* =\left\{\begin{array}{ll}
% \mathcal{O}\left(\frac{1}{k^{2-2\alpha}}\right)& \text{ if }\alpha \in \left( \frac{3}{4} , 1\right)\\
%\mathcal{O}\left( \frac{1}{\ln(k)^2}\right) & \text{ if } \alpha = 1.
%\end{array}\right.
%\end{eqnarray*} 
\begin{multline*}
\mathbb{E}[f(x_k)] - f^*\\
 =\left\{\begin{array}{ll}
 \frac{ \frac{(1-\alpha)^2}{c^2}E_0 +\frac{ c^2(4\alpha -2)\sigma^2}{4\alpha -3}}{(k^{1-\alpha} -1)^2}, & \alpha \in \left( \frac{3}{4} , 1\right)\\
 \frac{ \frac{1}{16c^2}E_0 + c^2 (1 +\ln(k))\sigma^2}{(k^{1/4} -1)^2}, &  \alpha =\frac{3}{4}.
\end{array}\right.
\end{multline*}
\end{proposition}


\begin{remark}
Since in \eqref{eq: values a_i and b_i acc Convex}, the parameters do not depend on $L$, we observe that the rate of convergence of $\mathbb{E}[f(x_k)] - f^*$ in the previsous proposition does not depend on the smoothness of $f$ and is accelerated compared to SGD (Proposition \ref{prop: decrease expectation E_k gd}).
\end{remark}

==> sections/N2N_NoAcc_Proofs.tex <==
\section{Proofs from Non-Accelerated Part}\label{Sec:ProofNoAcc}


\blue{ Maybe move this proof down } 
\begin{proof}[Proof of Theorem~\ref{Thm:ConvexLiapNoAcc}]
We will also prove the rates:
\begin{align}
\label{est_GD_1}
		f(x(t))-\minf &\leq \frac 1 {2t} |x_0-\minx|^2
\\
\label{GD_convex_rate2}
	f(x_k) - \minf &\leq \frac{1}{2hk} |x_0 -\minx|^2
\end{align}


[Proof of The convex part]

\blue{still need the strongly convex part}\\

Let $E(x,t) = E^c(x,t)$ be given by \eqref{Liap_GD}.  Then 
\begin{align}
\frac d{dt} E(x(t),t) 
&= - t |\nabla f(x)|^2 + f(x)-\minf  - (x-\minx)\cdot \nabla f(x) \\
 &\leq -t| \nabla f(x)|^2 && \text{by convexity of $f$} 
\end{align}
so \eqref{abstractLIAP} holds. 	Thus
\[
E(x(t),0) \leq E(x(0),0) = \frac 1 2 |x(0)-\minx|^2
\]
and
\begin{equation}\label{GD-stronger}
f(x(t))-\minf \leq \frac 1 {2t} \left( |x_0-\minx|^2 -  |x(t)-\minx|^2 \right) 	
\end{equation}
which gives~\eqref{est_GD_1}.

Next consider \eqref{abstractFE}, write $q_k = |x_k - \minx |^2/2$  and compute
\begin{align}
	E_{k+1}-E_k &= t_{k+1}(f_{k+1}-\minf) -t_{k}(f_{k}-\minf) + q_{k+1} - q_k\\
	&= t_{k+1}(f_{k+1}-f_{k})+ q_{k+1} - q_k + h(f_{k}-\minf)\\
	& \leq t_{k+1}\left ( \nabla f(x_k)(x_{k+1}-x_k) + \frac L 2 |x_{k+1}-x_k|^2  \right ) \\&+ \nabla q_k (x_{k+1}-x_k) + \frac 1 2 |x_{k+1}-x_k|^2  + h(f_{k}-\minf)
\end{align}	
where we have used convexity/smoothness for both $f$ and $q$.   Now use \eqref{abstractFE}
\begin{align}
	E_{k+1}-E_k 
	& \leq t_{k+1}h (-|v_k|^2) + t_{k+1}\frac{h^2 L}{2} |v_k|^2 + \frac{h^2}{2} |v_k|^2 + h(\nabla q_k v_k + f_k - \minf)\\
	&\leq \left ( -2t_{k+1}    + Lh t_{k+1} +h   \right ) \frac{ h|v_k|^2 }2 && \text{drop last term $f$ convex}\end{align}	
Using $t_k = kh$ and $h \leq 1/L$ gives 
\[
	E_{k+1}-E_k \leq 0
\]
so $h \leq 1/L$ gives the correct sign.	  The estimate \eqref{GD_convex_rate2} follows. 
\end{proof}


==> sections/N2N_SGD_NoAcc_SC.tex <==




\section{Gradient Descent NO ACC SC}
\begin{definition}\label{def:GD}
Define the continuous time gradient descent ordinary differential equation
\begin{equation}
	\label{GD-ODEsc}\tag{GD-ODE}
	\dot x(t) = - \nabla f(x(t))
\end{equation}
along with initial value $x(0) = x_0$.
Define the discrete time gradient descent
\begin{equation}\label{GD}\tag{GD}
	\frac{x_{k+1}-x_k}{h} = v(x_k) = -\nabla f(x_k)
\end{equation}
which is simply the explicit Euler time discretization \eqref{FE} of \eqref{GD-ODEsc}.

Then $\mu_E = L_E = 1$. 
\end{definition}

Our results in continuous and discrete time depend on the following simple estimate. 

\begin{lemma}
Suppose $f$ is $\mu$-strongly convex, and $x(t)$, $E(x)$, $v(x)$ are defined as in Definition~\ref{def:GD}.  Then 
	\begin{equation}\label{Esc-gd-estimate}
		\nabla_x E(x)\cdot v(x) \leq  - \left ( \mu E(x) + \frac 1 {2L} |v|^2\right ) 
	\end{equation}
In particular, $E$ is a rate-generating Liapunov function for $v$ with
\begin{align}
	a_E &= \frac{1}{2L} 
	&
	L_E &= 1
	&
	r_E &= \mu_f 
\end{align}


\end{lemma}
\begin{proof}
\begin{align}
	\nabla_x E(x)\cdot v(x) &= (x-\minx)\cdot(-\nabla f(x))\\
	&\leq \minf - f(x) - \mu \frac{|x-\minx|^2}{2} && \text{ by strong convexity \eqref{f_mu_strongly_convex_gen} }
\\
	& \leq -\frac{1}{2L} |\nabla f(x)|^2 - \mu E(x) && \text{ by \eqref{Gradf2_estimate} and \eqref{E_defn} }
\end{align}
which is \eqref{Esc-gd-estimate}.
\end{proof}

Now we can apply the general results on Liapunov functions from the previous section.




\begin{lemma}[Convergence rates for Gradient Descent]\label{lem_rate_GD}
	Suppose $f$ is $\mu$-strongly convex and $x(t)$ is the solution of \eqref{GD-ODEsc}.
	Then 
	\begin{equation}
		E(x(t)) \leq \exp(-\mu t) E(x_0)
	\end{equation}
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
	Suppose $f$ is $\mu$-strongly convex and $L$-smooth.
If
	\begin{equation}
		\label{CFL_strong_convex}\tag{CFL}
		h \leq \frac 2 {L}
	\end{equation}
then $E_k$ is decreasing at the rate 
	\begin{equation}\label{Rate_GD_convex0}
		E_k \leq \left(1- h \mu \right )^k E_0
	\end{equation}	
In particular, when equality holds in \eqref{CFL_strong_convex}, 
	\begin{equation}\label{Rate_GD_convex}
		|x_k-\minx|^2 \leq \left(1-\frac {2\mu} {L}\right )^k |x_0-\minx|^2
	\end{equation}	
\end{lemma}

\begin{proof}
Follows from \autoref{lem:FEconvergenceLIAP}
\end{proof}



\subsection{SGD no ACC Strongly convex case: continuous and discrete time}
\label{Appendix: SGD-SC}

Let us study the equation 
%
\begin{eqnarray}
\label{eq: perturbed gradient descent strongly convex}
\dot{x} = - (\nabla f(x) +e(t)), 
\end{eqnarray}
for an error function, $e$ satisfying 
%
\begin{eqnarray}
\label{ass: integrability e SGD}
\int_0^{+\infty} e^{\mu s} |e(s)| \, ds < +\infty.
\end{eqnarray}
This condition on the error function is classical \cite{Robbins}.  The case $e=0$ is satisfied trivially and corresponds to the gradient descent ODE. 


We define the function $E \, : \, [0,+\infty )  \times {\R}^d \rightarrow [0,+\infty )$ by
%
$$ E(t,x) = \frac{1}{2}|x-x^*|^2 + I(t),$$
%
where,
%
$$ I(t) = e^{-\mu t} \int_0^t e^{\mu s} \langle x(s) - x^*, e(s) \rangle \, ds.$$

Then we have the following result.

\begin{proposition}
\label{prop: rate SGD strongly convex}
Let $x$ be a solution of \eqref{eq: perturbed gradient descent strongly convex} with initial data $x_0$ and suppose that $e$ satisfies \eqref{ass: integrability e SGD}. Then,
%
$$ \frac{d E(t,x)}{dt} \leq -\mu E(t,x).$$
%
In addition, $\sup_{t\geq 0} |x - x^*| < +\infty$ and 
%
$$ \frac{1}{2}|x-x^*|^2 \leq e^{-\mu t} \left( \frac{1}{2}|x_0 -x^*|^2 + \sup_{s \geq 0} |x(s) -x^*|\int_0^{+\infty} e^{\mu s} |e(s) | \,ds \right).$$

\end{proposition}

\begin{proof}
For all $t>0$, 
%
\begin{eqnarray*}
 \frac{d E(t,x)}{dt} & =  &- \langle x - x^*, \nabla f(x) \rangle -   \langle x - x^*, e \rangle - \mu I(t) +\langle x - x^*, e \rangle\\
 &\leq & - \frac{\mu}{2}|x -x^*|^2 - \mu I(t) = -\mu E(t,x).
\end{eqnarray*}
%
Therefore $E(t,x(t))$ is decreasing and then for all $t>0$,
%
$$ \frac{1}{2}|x(t) - x^* | ^2 \leq \frac{1}{2} |x_0 -x^*| + \int_0^t |x(s)-x^*| e^{\mu s} |e(s)| \,ds.$$
%
By Gronwall Lemma and \eqref{ass: integrability e SGD}, we deduce that $\sup_{t\geq 0} |x - x^*| < +\infty$ and the proof is concluded.
\end{proof}


The discretization of \eqref{eq: perturbed gradient descent strongly convex} is 
%
$$ x_{k+1} - x_k = -h (\nabla f(x_k) +e_k),$$
%
where $e_k=e(hk)$. We define $E_k$, for $k \geq 1$, by 
%
$$ E_k = \frac{1}{2}|x_k -x^* |^2 + I_k,$$
%
where,
%
$$ I_k= (1 - h\mu)^k h\sum_{i=0}^k (1 - h\mu)^{-i} \langle x_i -x^*, e_{i-1} \rangle,$$
%
with the notation $e_{-1}=0$.


\begin{proposition}
Assume that $h \leq \frac{1}{L}$. Then,
%
$$ E_{k+1} -E_k \leq - h\mu E_k.$$
%
In addition, if the sequence $(1 - h\mu)^{-i}|e_i|$ is summable, $\sup_{i\geq 1} |x_i -x^*| < +\infty$ and we deduce,
%
$$ \frac{1}{2}|x_k - x^*|^2 \leq (1 -h\mu)^k \left( \frac{1}{2}|x_0 -x^*|^2 + h\sup_{i\geq 1} |x_i -x^*| \sum_{i=0}^{+\infty} (1 - h\mu)^{-i-1} |e_{i} | \right).$$

\end{proposition}

\begin{proof}
First, as usual, we have
%
\begin{eqnarray*}
\frac{1}{2}|x_{k+1} - x^*|^2 -\frac{1}{2}|x_{k} - x^*|^2 & =&  -h\langle \nabla f(x_k) ,x_k -x^* \rangle - h \langle e_k ,x_k -x^* \rangle + \frac{h^2}{2} |\nabla f(x_k) +e_k|^2\\
&\leq & -\frac{h\mu }{2} |x_k -x^* |^2 +h(f^* -f(x_k))+ \frac{h^2}{2} |\nabla f(x_k) +e_k|^2\\
&\leq & -\frac{h\mu }{2} |x_k -x^* |^2 -\frac{h}{2L}|\nabla f(x_k) |^2 + \frac{h^2}{2} |\nabla f(x_k) +e_k|^2.
\end{eqnarray*}
%
In addition,
%
\begin{eqnarray*}
I_{k+1} - I_k &=& h(1-h\mu )^k \left( (1- h\mu)\sum_{i=0}^{k+1} (1-h\mu)^{-i}\langle x_i -x^*, e_{i-1} \rangle - \sum_{i=0}^{k} (1-h\mu)^{-i}\langle x_i -x^*, e_{i-1}\rangle \right)\\
& = & -h \mu I_k + h \langle x_{k+1} -x^*, e_k \rangle.
\end{eqnarray*}
%
Combining these two inequalities,
%
\begin{eqnarray*}
E_{k+1} -E_k &\leq & -h \mu E_k +h \langle x_{k+1} -x_k, e_k \rangle  -\frac{h}{2L}|\nabla f(x_k) |^2 + \frac{h^2}{2} |\nabla f(x_k) +e_k|^2\\
& \leq & -h \mu E_k + \frac{h}{2}\left(h -\frac{1}{L} \right) |\nabla f(x_k) |^2 -\frac{h^2}{2}|e_k|^2\\
& \leq &  -h \mu E_k,
\end{eqnarray*}
%
when $h \leq \frac{1}{L}$.\\

In order to conclude, we also need to establish that $E_k$ is bounded below.  That follows from discrete Gronwall's inequality, as was already done in the continuous case in Proposition \ref{prop: rate SGD strongly convex}.
\end{proof}




==> sections/N2N_abstract_lyap.tex <==
\section{Abstract Lyapunov Analysis: going from continuous to discrete time}
\label{section: abstract Liap}


In this section we present an abstract analysis showing how to go from deterministic continuous time to stochastic discrete time. We make a definition of the continuous problem and start exposing the problem in an abstract setting. Then, we show how this framework can be extended to study the stochastic case. We  introduce abstract assumptions (e.g inequalities \eqref{ass: lyap discrete abstract}, \eqref{ass: expectation E_k r_E=0 1} and \eqref{ass: expectation E_k r_E=0 2}) which are easily verified in the gradient case. These assumptions are later proven in the accelerated case.



\subsection{ODEs, Perturbed ODEs and discretizations}
\begin{definition}
\label{def: def abstract ODE and g}
Let $g(t,z,p)$ be $L_g$-Lipschitz continuous, and affine in the variable $p$,
\begin{equation}\label{g_affine}
	g(t,z,p) = g_1(t,z) + g_2(t,z) p.
\end{equation}
Consider the Ordinary Differential Equation 
\begin{align}
\label{abstractODE}\tag{ODE}
	\dot{z}(t) &= g(t,z(t),\nabla f(z(t)) )
\end{align}
Referring to \eqref{perturbed_gradient}, 
Consider also the perturbed ODE, 
\begin{equation}
\label{ODE sto}\tag{PODE}
	\dot{z}(t) = g(t, z(t), \tilde \nabla f(z(t)) ).
\end{equation}
\end{definition}
\eqref{abstractODE}  has unique solutions in all time for every  initial condition $z(0) = z_0 \in \R^n$. 
Moreover, if we assume that $e(t)$ is Lipschitz continuous in time, then \eqref{ODE sto} has unique solutions in all time for every initial condition $z(0) = z_0 \in \R^n$.   On the other hand, if we wish to consider a model of $e(t)$ which is more consistent with random, mean zero errors, then \eqref{ODE sto} is no longer well-posed as an ODE.  However, we can consider a Stochastic Differential Equation (\cite{oksendal2013stochastic,pavliotis2016stochastic}), which would lead to similar results to the discrete case where we take expectations of the mean zero error term.   We do not pursue the SDE approach here to simplify the exposition. 

\begin{definition}
For a given learning rate schedule $h_k \geq 0$ and $t_k = \sum_{i=0}^k h_i$, the forward Euler discretization of  \eqref{abstractODE} corresponds to the sequence 
\begin{equation}\label{abstractFE}\tag{FE}
	z_{k+1} = z_k + h_k g(t_k,z_k,\nabla f(z_k)), 
	%\qquad  	t_k = \sum_{i=0}^k h_i  
\end{equation}
given an initial value $z_0$. 
Similarly, the forward Euler discretization of  \eqref{ODE sto} is given by 
\begin{equation}
\label{abstractFE sto}\tag{FEP}
	z_{k+1} = z_k + h_k g(t_k,z_k,\nabla f(z_k) +e_k) 
\end{equation}
\end{definition}


The solution of \eqref{abstractFE} or of  \eqref{abstractFE sto} can be interpolated to be a function of time  $z^h : [0,T) \to \R^n$ by simply setting $
z^h(t_k) = z_k$ along with piecewise constant or piecewise linear interpolation between time steps. It is a standard result from numerical analysis of ODE  theory~(\cite{iserles2009first}) that functions $z^h$ converge to $z(t)$ with error of order $h_k$, provided $h_k \leq 1/L_g$. 

\subsection{Lyapunov analysis for the unperturbed ODE}
First, we give the definition of a rate-generating Lyapunov function for \eqref{abstractODE}. 
\begin{definition}
\label{def:reate-gene Lyap abstract}
 We say $E(t,z)$ is a rate-generating Lyapunov function for \eqref{abstractODE} if, for all $t>0$, $E(t,z^*)=0$ and $\nabla E(t,z^*)=0$ where $z^*$ is a stationary solution of \eqref{abstractODE}, i.e. $g(t,z^*, \nabla f(z^*) )=0$, and if there are constants $r_E , a_E  \geq 0$ such that 
\begin{multline}\label{Liap_Cond}
 \partial_t E(t,z) + \nabla E(t,z) \cdot g(t,z, \nabla f(z) )
  \leq -  r_E E(t,z) - a_E |g(t,z,\nabla f(z))|^2 
\end{multline}
\end{definition}
%
\begin{remark}
We use a similar definition which is used in the convex case, where now
$r_E = 0$ and the constant $a_E$ is extended to be a function of time $a_E(t)$. The analysis below does not change. 
\end{remark}


Then, we can deduce the following rate in the continuous case.
%
\begin{lemma}
\label{lem: abstrat ODE no acc}
Let $E$ be a rate generating Lyapunov function for \eqref{abstractODE}. 
Then 
\[
E(t,z(t)) \leq E(0,z(0)) \exp(-r_E t)
\]
\end{lemma}
\begin{proof}
%\red{notation: gradient $\nabla E$ means gradient in $z$ variable}
\begin{multline*}
		\frac{d}{dt}E(t,z(t))  
		= \partial_t E(t,z(t)) + \nabla E(t,z(t)) \cdot g(t,z(t), \nabla f(z(t)) ) \\
		\leq - r_E E(t,z(t)) - a_E |g(t,z(t),\nabla f(z(t)))|^2 
\end{multline*}
by assumption \eqref{Liap_Cond}. Gronwall's inequality gives the result.
\end{proof}
%





\subsection{Dissipation of $E$ along \eqref{abstractFE sto}}

Now we consider the discrete case where $\nabla f$ has been replaced by a perturbed gradient $\tilde{\nabla }f = \nabla f +e$ and then we compute the dissipation of $E$ along \eqref{abstractFE sto}.

First, we assume, in addition, there exists $L_E > 0$ such that $E$ satisfies,
	\begin{multline}
	\label{ass: lyap discrete abstract}
	E(t_{k+1},z_{k+1}) - E(t_k,z_k) 
	\leq \partial_t E(t_k,z_k) (t_{k+1}-t_k) \\
	+\langle \nabla E(t_k,z_k) , z_{k+1}- z_k \rangle 
	+\frac{L_E}{2} |z_{k+1}-z_k|^2.
	\end{multline} 


\begin{lemma}
\label{lem:abstract dissipation E_k perturbed}
Let $z_k$ be the solution of \eqref{abstractFE sto}.  
Suppose $E$ is a rate-generating Lyapunov function for \eqref{abstractODE} which satisfies \eqref{ass: lyap discrete abstract}.  Then if $h_k$ satisfies
\begin{equation}
\label{ass: abstract CFL}
h_k \leq \frac{2a_E}{L_E},
\end{equation}
we have
\begin{equation}\label{Ek_change_perturbed}
	E(t_{k+1}, z_{k+1}) - E(t_k,z_k) \leq  -h_k r_E E(t_k,z_k) + h_k \beta_k 
\end{equation}
where $\beta_k$ is defined by 
\begin{multline}
\label{beta_i_defn}
\beta_k := \left\langle \nabla E(t_k,z_k), g_2(t_k,z_k)e_k \right\rangle \\
 +L_E h_k\left\langle g(t_k,z_k,\nabla f(z_k)) + \frac{1}{2}g_2(t_k,z_k)e_k , g_2(t_k,z_k)e_k \right\rangle.
\end{multline}
\end{lemma}

%\begin{remark}
%	Note \eqref{Ek_change_perturbed} is a perturbation of the analogous result in the continuous case: the first term in $\beta_k$ is a discretization of the corresponding term in the continuous case - the remaining terms are perturbations of order $h$. 
%\end{remark}

%\begin{remark}
%	Note also that if under the standard assumptions on the error, $\mathbb{E}[ e_i ] = 0$ and $Var(e_i) = \sigma^2$, along with independence, then 
%	\begin{equation}
%		\mathbb{E}[ \beta_k ] = h \frac{L_E g_2^2}{2} \sigma^2
%	\end{equation}
%\end{remark}




\subsection{Convergence in expectation: $r_E > 0$}
\label{subsection: abstract variable time step}
Now we consider the case where the error $e_k$ satisfies \eqref{ass: mean and varience error}.
We require that $h_k$ satisfies \eqref{ass: abstract CFL}.
(This assumption is easy to enforce, since, in practice, we can perform a few steps of the algorithm, and reset, so that until $h_k$ small enough).
%\red{change here, please confirm} 
We consider the case $r_E > 0$, which applies to the strongly convex case.

By definition of $\beta_k$,
\[
\mathbb{E}[\beta_k ]  = \frac{h_k L_E g_2(t_k, z_k)^2 \sigma^2}{2},
\]
and then, taking the expectation in \eqref{Ek_change_perturbed}, we obtain
\begin{equation}
	\label{eq: expectation E_k}
\mathbb{E}[E(t_{k+1},z_{k+1})]  
\leq (1 - h_k r_E) E(t_{k},z_{k}) + \frac{h_k^2 L_E g_2(t_k, z_k)^2 \sigma^2}{2}.  
\end{equation}

Then, we deduce the following result
\begin{proposition}[Case $r_E>0$]
\label{prop: decrease expectation E_k}
Assume that $r_E>0$ and $\overline{g_2} = \max_{(t,z)} g_2(t,z) <+\infty$. If
\[
h_k := \frac{2}{r_E (k +\alpha^{-1} E_0^{-1}) } \qquad \text{where } \qquad \alpha=\frac{r_E^2}{2L_E\overline{g_2}^2 \sigma^2},
\]
then,
\begin{equation}
\label{eq: decrease expectation E_k}
\mathbb{E}[E(t_{k},z_{k})] \leq \frac{1}{\alpha(k + \alpha^{-1} E_0^{-1})}.
\end{equation}
\end{proposition}



\subsection{Convergence in expectation: $r_E = 0$}
Since the convex case corresponds to  the $r_E=0$ case, the rate of convergence has to be incorporated into the Lyapunov function. Then we assume that there exists five constants $a_1,a_2,a_3,b_1,b_2\geq 0$ such that
  \begin{equation}
  \label{ass: expectation E_k r_E=0 1}
\mathbb{E}[E(t_{k+1},z_{k+1})]  -E(t_{k},z_{k})\leq  \frac{  (a_1  + a_2t_k +a_3t_k^2) h_k^2\sigma^2}{2}
  \end{equation}
  and in addition, that 
   \begin{equation}
  \label{ass: expectation E_k r_E=0 2}
 \mathbb{E}[E(t_{k},z_{k})] \geq  (b_1t_k + b_2t_k^2) ( \mathbb{E}[f(x_k)] - f^*).
  \end{equation}
We will see below that these conditions are easily verified in the non-accelerated case, and that it also holds for the accelerated case. Then we obtain
  %
 \begin{proposition}
\label{prop: decrease expectation E_k r_E=0}
Assume that $r_E=0$ and \eqref{ass: expectation E_k r_E=0 1}-\eqref{ass: expectation E_k r_E=0 2} hold. If $h_k = \frac{c}{k^{\alpha}}$, $t_k =\sum_{i=1}^k h_i$, then the following holds:
\begin{itemize}
\item Case $a_1,a_2,b_1>0$, $a_3=b_2=0$: If $\alpha \in \left[ \frac{2}{3} , 1\right)$, then 
%\begin{eqnarray*}
%\mathbb{E}[f(x_k)] - f^* =\left\{\begin{array}{ll}
% \mathcal{O}\left( \frac{1}{k^{1-\alpha}}\right) & \text{ if }\alpha \in \left( \frac{2}{3} , 1\right)\\
% \mathcal{O}\left( \frac{1}{\log(k)}\right) & \text{ if } \alpha = 1.
%\end{array}\right.
%\end{eqnarray*} 
\[
\mathbb{E}[f(x_k)] - f^*
 \leq \left\{\begin{array}{ll}
 \dfrac{ \dfrac{1-\alpha}{c}E_0 +\left(\dfrac{a_1  c(1- \alpha)\alpha }{2\alpha -1} +\dfrac{a_2  c^2(3\alpha -1)}{2(3\alpha -2)}\right) \sigma^2}{b_1(k^{1-\alpha} -1)}, & \alpha \in \left( \dfrac{2}{3} , 1\right)\\
\dfrac{ \dfrac{1}{3c}E_0 +\left(\dfrac{2a_1  c}{3}+\dfrac{a_2  c^2 }{2}(1+\log(k))\right) \sigma^2}{b_1(k^{1/3} -1)} , &  \alpha = \dfrac{2}{3}.
\end{array}\right.
\]
\item Case $a_1=a_2=b_1=0$, $a_3>0$ and $b_2> 0$: If $\alpha \in \left[ \frac{3}{4} , 1\right)$, then 
%
%\begin{multline*}
%\mathbb{E}[f(x_k)] - f^*\\
% =\left\{\begin{array}{ll}
% \mathcal{O}\left(  \frac{b_1}{k^{1-\alpha}} + \frac{b_2}{k^{2-2\alpha}}\right) & \text{ if }\alpha \in \left( \frac{3}{4} , 1\right)\\
% \mathcal{O}\left( \frac{b_1}{\log(k)} + \frac{b_2}{\log(k)^{2}}\right) & \text{ if } \alpha = 1.
%\end{array}\right.
%\end{multline*}
%\end{itemize} 
\[
\mathbb{E}[f(x_k)] - f^*
\leq \left\{\begin{array}{ll}
 \dfrac{ \dfrac{(1-\alpha)^2}{c^2}E_0 +\dfrac{a_3  c^2(4\alpha -2)\sigma^2}{2(4\alpha -3)}}{b_2(k^{1-\alpha} -1)^2}, & \alpha \in \left( \dfrac{3}{4} , 1\right)\\
 \dfrac{ \dfrac{1}{16c^2}E_0 +\dfrac{a_3  c^2 \sigma^2}{2}(1 +\log(k))}{b_2(k^{1/4} -1)^2}, &  \alpha =\dfrac{3}{4}.
\end{array}\right.
\]
\end{itemize} 
\end{proposition}

%We will see that this result can be applied for convex gradient descent and convex accelerated gradient method.







==> sections/N2N_applications.tex <==
\section{Application to gradient descent}
\label{section:application}
In this section, we apply our previous abstract analysis to gradient descent for convex and strongly convex functions. In this case, $g$ from \eqref{g_affine} is simply given by 
\[
g(t,z,p) = -p
\]
%
Let $f$ be a $\mu$-strongly convex, $L$-smooth function. Consider
%
\begin{equation}
\label{eq: GD}
\dot{x}(t) = -\nabla f(x(t)) 
\end{equation}
and its associated perturbed forward Euler scheme, where the gradient is replaced by $\tilde{\nabla }f = \nabla f +e$ 
\begin{equation}
\label{eq: dicrete SGD convex}
x_{k+1} -x_k  = - h_k( \nabla f(x_k) +e_k),
\end{equation}
with initial condition $x_0$.
Define the  convex and strongly convex Lyapunov functions 
\begin{equation}
	\label{EGD}
	\begin{aligned}
	E^c (t,x) &:= t(f(x) -f^*) +\frac{1}{2}|x-x^*|^2,\\
	E^{sc} (x) &:= f(x) -f^* + \frac{\mu}{2}|x-x^*|^2.
\end{aligned}
\end{equation}

\subsection{Continuous analysis}

First, we show that the Lyapunov functions satisfy \eqref{ass: lyap discrete abstract}.
%
\begin{proposition}
\label{lem: condition GD lyapunov function}
\begin{itemize}
\item $E^c$ is a Lyapunov function in the sense of Definition \ref{def:reate-gene Lyap abstract} with $r_{E^c} =0$ and $a_{E^c}=t$. In addition, $E^c$ satisfies \eqref{ass: lyap discrete abstract} with $L_{E^c}= Lt_{k+1} +1$.


\item $E^{sc}$ is a Lyapunov function in the sense of Definition \ref{def:reate-gene Lyap abstract} with $r_{E^{sc}} =\mu$ and $a_{E^{sc}}=1$. In addition, $E^{sc}$ satisfies \eqref{ass: lyap discrete abstract} with $L_{E^{sc}}= L+\mu$.
\end{itemize}

\end{proposition}




Applying Lemma \ref{lem: abstrat ODE no acc} to $E^c$ and $E^{sc}$, we  recover the usual rates. 
\begin{corollary}
Let $x$ be the solution of \eqref{eq: GD}. Then, for all $t \geq 0$,
\[\begin{array}{ll}
f(x(t))-\minf \leq \frac 1 {2t} |x_0-\minx|^2 & \text{(cvx)}\\
\\
f(x(t)) -f^* +\frac{\mu}{2}|x(t) -\minx|^2 \leq e^{-\mu t} E^{sc}(x_0) & \text{(st. cvx)}
\end{array}
\]
%\begin{itemize}
%\item Convex case: for all $t \geq 0$,
%\begin{equation}
%f(x(t))-\minf \leq \frac 1 {2t} |x_0-\minx|^2,
%\end{equation}
%%
%\item Strongly convex case: for all $t \geq 0$,
%\begin{equation}
%f(x(t)) -f^* +\frac{\mu}{2}|x(t) -\minx|^2 \leq e^{-\mu t} E^{sc}(x_0).
%\end{equation}
%\end{itemize}

\end{corollary}



\subsection{Perturbed gradient descent} \label{Appendix: SGD}
In the case where the gradient is replaced by a perturbed gradient $\tilde{\nabla } f = \nabla f + e$, where $e$ is an error term, by Lemma \ref{lem: abstrat ODE no acc}, the dissipation of $E^c$ and $E^{sc}$ along \eqref{eq: dicrete SGD convex} is given in the next proposition.
%
\begin{proposition}
\label{prop: dissipation GD perturbed convex str convex}
Let $x_k$ be the sequence generated by perturbed gradient descent \eqref{eq: dicrete SGD convex}.
%
\begin{itemize}
\item Convex case: If $h_k$ satisfies, $h_k \leq \frac{1}{L}$,
%\begin{equation}
%	\label{ass: time step discrete SGD convex}
%h_k \leq \frac{1}{L},
%\end{equation} 
and $t_k = \sum_{i=0}^k h_i$, then, $E^c_k$ satisfies 
\begin{equation}
\label{eq: main eq convex GD time variable}
E^c_{k+1} \leq E^c_k + h_k\beta_k^c,
\end{equation}
where $ \beta_k^c := -\langle x_k - x^* -t_{k+1} \nabla f(x_{k}) , e_{k} \rangle 
 + h_k(Lt_{k+1} +1)\left\langle  \nabla f(x_k) + \frac{1}{2}e_k, e_k \right\rangle$.
%
\item Strongly convex case: If $h_k$ satisfies $h_k \leq \frac{2}{L+\mu}$, %$ h_k \leq \frac{2}{L+\mu}$, then
%\begin{equation}
%	\label{ass: time step discrete SGD str convex}
%h_k \leq \frac{2}{L+\mu}.
%\end{equation}
then, $E^{sc}_k$ satisfies 
\begin{equation}
\label{eq: main eq str convex GD time variable}
E^{sc}_{k+1} \leq (1-h_k\mu ) E^{sc}_k + h_k\beta_k^{sc},
\end{equation}
where $ \beta_k^{sc}=\langle \mu(x_k -x^*) + \nabla f(x_k)  , e_k \rangle 
  +h_k(L+\mu) \left\langle\nabla f(x_k) +\frac{1}{2}e_k , e_k \right\rangle.$
\end{itemize}
\end{proposition}


\subsection{Variable time step and convergence in expectation}
Now, consider the case of a variable time step $h_k$ and a zero-mean and fixed Variance error $e_k$ i.e. $e_k$ satisfies \eqref{ass: mean and varience error}. From Proposition \ref{prop: dissipation GD perturbed convex str convex}, since $\mathbb{E}[\beta_k^{c}] = \frac{h_k^2(Lt_{k+1} +1)\sigma^2}{2}$ and $ \mathbb{E}[\beta_k^{sc}] = \frac{h_k^2(L +\mu)\sigma^2}{2}$, 
\begin{eqnarray*}
\mathbb{E}[E^c_{k+1}] &\leq & E^c_k  + \frac{h_k^2(Lt_{k+1} +1)\sigma^2}{2} \\
\mathbb{E}[E^{sc}_{k+1}] &\leq & (1- \mu h_k)E^{sc}_k  + \frac{h_k^2(L+\mu)\sigma^2}{2}.
\end{eqnarray*}
In addition,  
\[
\mathbb{E}[E^c_{k}] \geq t_k ( \mathbb{E}[f(x_k)] -f^*) ,
\]
which correpsond, for $E_k^c$, to \eqref{ass: expectation E_k r_E=0 1} and \eqref{ass: expectation E_k r_E=0 2} with 
\[
a_1 =\frac{L(h_k +1)}{2},\, a_2 =\frac{L}{2}, \, a_3 =0, \, b_1= 1 \text{ and } b_2 =0.
\]
And, for $E_k^{sc}$, to the case where $r_{E^{sc}}= \mu>0$ and $g_2^2= 1$, then Proposition \ref{prop: decrease expectation E_k} and Proposition \ref{prop: decrease expectation E_k r_E=0} give:

\begin{proposition}
\label{prop: decrease expectation E_k gd}
%Assume that $E^c_0= E^{sc}_0=E_0$.% satisfies \eqref{ass: time step discrete SGD convex} and \eqref{ass: time step discrete SGD str convex}.
\begin{itemize}
\item Convex case ($r_{E^c}=0$):
If $h_k^{c} := \frac{c}{k^{\alpha}}$ satisfies $h_k^{c} \leq \frac{1}{L}$, and $t_k =\sum_{i=1}^k h_i^c$, then the following holds:
%\begin{eqnarray*}
%\mathbb{E}[f(x_k)] - f^* =\left\{\begin{array}{ll}
% \mathcal{O}\left(\frac{1}{k^{1-\alpha}}\right)& \text{ if }\alpha \in \left( \frac{2}{3} , 1\right)\\
%\mathcal{O}\left( \frac{1}{\ln(k)}\right) & \text{ if } \alpha = 1.
%\end{array}\right.
%\end{eqnarray*} 
\[
\mathbb{E}[f(x_k)] - f^*
 \leq \left\{\begin{array}{ll}
 \dfrac{ \dfrac{1-\alpha}{c}E_0 +\dfrac{Lc^2(3\alpha - 1)\sigma^2}{2(3\alpha -2)}}{k^{1-\alpha} -1}, & \alpha \in \left( \dfrac{2}{3} , 1\right)\\
\dfrac{ \dfrac{1}{3c}E_0 +\left( 3c +Lc^2(1+ \ln(k) \right) \dfrac{\sigma^2}{2}}{k^{1/3} -1}, &  \alpha = \dfrac{2}{3}.
\end{array}\right.
\]
\item Strongly convex case ($r_{E^{sc}}=\mu>0$): If
 \[ h_k^{sc} := \frac{2}{\mu (k + (\alpha^{sc}E_0^{sc})^{-1})}, \, \, \alpha^{sc} := \frac{\mu}{2(C_f+1)\sigma^2}\] 
 and $t_k =\sum_{i=0}^k h_i$, 
 then, if $h_k^{sc}$ satisfies $h_k^{sc} \leq \frac{2}{L+\mu}$, the following holds:
\[
\mathbb{E}[E(x_k)] \leq \frac{2(C_f +1) \sigma^2}{\mu k + 2(C_f +1) \sigma^2 {E_0^{sc}}^{-1}}.
\]
\end{itemize}
\end{proposition}




==> sections/N2N_numerics.tex <==
\section{Numerical simulations}
\label{section: simulations}


\begin{figure}
\begin{center}
\includegraphics[ scale=0.3]{Figures/FigureBound}
\end{center}
\caption{Constant time step algorithms for SGD and accelerated SGD in the strongly convex case.  SGD reaches a value below the bound (blue dotted line) at an an exponential rate: accelerated SGD reaches a value below the bound (red dotted line) at an accelerated exponential rate.  The theory holds but is not sharp: SGD reaches a lower value.}
\label{figureAGD}
\end{figure}

\red{TO DO}

\subsection{Effect of $v$ on $x$?}


\red{Plot of convergence of $x$ and $v$ (full and stochastic cases)?}




\subsection{Comparison and discussion}

\paragraph{\textbf{Algorithm in the convex case:}}  Analysis will give the best constant, and yield the following algorithm (Proposition \ref{prop: modified Nesterov}): Define $h_k = \min\left(\frac{c}{k^{3/4}}, \frac{1}{\sqrt{L}}\right)$ and $t_k$ by
\[
t_k = \left\{\begin{aligned}
\frac{k+2}{\sqrt{L}} & \text{ if } k<k_0\\
t_{k_0 -1} + \sum_{i = k_0}^{k-1} \frac{c}{i^{3/4}}  & \text{ if } k \geqslant k_0,
\end{aligned} \right.
\]
where $k_0 = \lceil c^{3/4}L^{2/3} \rceil$. Note that $t_{k_0-1} \approx \frac{1+c^{3/4}L^{2/3} }{\sqrt{L}}$. Then, the scheme \eqref{eq: Nesterov like system} becomes

\begin{equation}
\label{eq: Nesterov like system}
\left\{
\begin{aligned}
		x_{k+1} &= y_k  - \frac{h_k}{\sqrt{L}}\nabla f(y_k)\\
   y_{k+1} & = x_{k+1} + \frac{h_{k+1} t_{k}}{h_{k} t_{k+1}}\left(1 - \frac{2h_k}{t_k}\right)(x_{k+1} - x_k) + \frac{ t_{k}}{ t_{k+1}}h_{k+1}\left( \frac{1}{h_k} - \sqrt{L} \right)(x_{k+1} - y_k).
\end{aligned}
\right . 
\end{equation}



\paragraph{\textbf{Algorithm in the strongly convex case:}} Analysis will give the best constant, and yield the following algorithm (Proposition \ref{prop: modified Nesterov}): Define $h_k = \min\left(\frac{2\sqrt{\mu}}{\mu k +4\sigma^2 \gamma^{-1} }, \frac{1}{\sqrt{L}}\right)$. Introducing
\[
\hat{k} := \left( k -  \left( 2\sqrt{C_f} - \frac{4\sigma^2}{\mu \gamma} \right) \right)_+, 
\]
the learning rate becomes
\[
h_k = \frac{1}{\sqrt{L}} \frac{2\sqrt{C_f}}{2\sqrt{C_f} +\hat{k}}.
\]

\red{\begin{remark}
If we want to be able to use the induction proof when $\hat{k}$ becomes positive, let say at $k_0$, we need to have $E_{k_0} \leq \gamma$. 
\end{remark}}


Then, the algorithm in Proposition \ref{prop: modified Nesterov} can be rewritte as
\begin{equation}
\label{eq: SC Nesterov like system}\tag{Pert-SC-Nest}
\left \{
\begin{aligned}
		x_{k+1} &= y_k  - \frac{2 \sqrt{C_f}}{2\sqrt{C_f} +\hat{k}} \frac{1}{L}\nabla f(y_k)\\
   y_{k+1} & = x_{k+1} + \left(\frac{2 (\sqrt{C_f} -1) +\hat{k}}{2 (\sqrt{C_f} +1) +\widehat{k+1}}\right)(x_{k+1} - x_k) -\left(\frac{\hat{k}}{2 (\sqrt{C_f} +1) +\widehat{k+1}}\right)(x_{k+1} - y_k).
\end{aligned}
\right . 
\end{equation}	


%\red{To do: rewrite sytem \eqref{eq: SC Nesterov like system} with the good $h_k$}

==> sections/n2n_intro_Old.tex <==
\section{Introduction}

%\subsection{List of changes by adam}
%\begin{enumerate}
%	\item change abstract from original AISTATS to newer one
%	\item Check for typos: section 4.3 second equation $t f - f*$ to $f(f-f^*)$. 
% \item elaborated on the proof of proposition 4.2
%\end{enumerate}
%
%TODO
%\begin{enumerate}
%	\item Remove the two ODEs, notation for perturbed, just in the first section.
%\end{enumerate}



Recently \citet{su2014differential} showed that Nesterov's method for accelerated gradient descent can be obtained as the discretization of an Ordinary Differential Equation (ODE).   The work of \cite{su2014differential} resulted in a renewed interest in the continuous time approach to first order optimization, for example \cite{wibisono2016variational, wilson2016lyapunov, wilson2019acceleration}.  The goals of the approach are to: (i) develop new insights into accelerated algorithms, and (ii) obtain new optimization algorithms.  However, so far there has limited progress made on the second goal.  

There is more than one ODE which can be discretized to obtain Nesterov's method~\citet{shi2018understanding}.  We show that Nesterov's method has a natural interpretation as a coupled system of two first order ODEs: the first is gradient descent with the usual learning rate, and the second is a gradient descent with a faster learning rate.  On it's own, the second equation is unstable, however, but coupling the two equations together, using a single parameter, we obtain an Nesterov's method.  Moreover, this system of ODEs decreases a Lyapunov function.  By choosing a decreasing learning rate, in the case of stochastic gradients, we obtain an accelerated stochastic gradient descent algorithm.  We prove, using a Lyapunov function approach,  that for both the convex and strongly convex cases, the algorithms converge at the optimal rate for the last iterate of SGD, with rate constants which are better than previously available.
By discretizing a specific choice of ODE, we show that: (i) with a constant learning rate, we obtain Nesterov's method, (ii) with a decreasing learning rate, we obtain an accelerated stochastic gradient descent algorithm. 




\subsubsection*{{Notation:}} 
Let $f$ be a proper convex function, and write  $\minx = \argmin_x f(x)$ and $\minf = f(\minx)$.  We say $f$ is $L$-smooth if 
\begin{align}
	\label{Basic_Lsmooth}
	f(y) - f(x) + \nabla f(x)\cdot(x-y) &\leq \frac L 2 |x-y|^2, 
%	&& \text{ for all } x,y \in \Rn .
\end{align} 
and $f$ is $\mu$-strongly convex if
\begin{equation}\label{f_mu_strongly_convex_gen}
	f(x) + \nabla f(x)\cdot(y - x) \leq f(y) -  \frac{\mu}{2}|x-y|^2,
%	\qquad \text{ for all } x,y \in \Rn .
\end{equation}
for all $x,y$ respectively.  Write $C_f := \frac{L}{\mu}$ for the condition number of $f$. 


\subsection{Stochastic gradient descent}
Stochastic gradient descent (SGD) is the iteration
\begin{equation}
	\label{tempSGD}
	x_{k+1} = x_k - h_k \widehat g(x_k)
\end{equation}
where $h_k$ is the learning rate, and $\widehat g(x_k)$ is an approximation to the gradient  $\nabla f(x_k)$. We study the stochastic approximation setting, meaning that we assume $\widehat g(x,\xi)$ is an unbiased estimator of the gradient $\nabla f(x)$, so that $\mathbb{E}[\widehat{g}(x,\xi)] = \nabla f(x)$, and that the variance is bounded $
\Var(\widehat{g}(x,\xi)) \leq \sigma^2$.  Write 
\begin{equation} \label{perturbed_gradient}
\widehat g(x,\xi)  = \nabla f(x) + e(x, \xi),
\end{equation}
%and make the stochastic approximation assumption on the error, 
where 
\begin{equation}
\label{ass: mean and varience error}
\mathbb{E}[e] = 0 \, \text{  and  } \, \Var(e) \leq \sigma^2.
%\mathbb{E}[ \|e\|^2]  \leq \sigma^2>0.
\end{equation}
 More general assumptions are discussed in \cite{bottou2018optimization}.  The assumption \eqref{ass: mean and varience error} allows us to express our convergence rates in terms of $\sigma^2$.   Relaxing the assumption \eqref{ass: mean and varience error} to cover the finite sum case is the subject of future work.  
The following fundamental inequality can be found in \cite{bottou2018optimization},
\begin{equation}
\label{eq: bottou inequality}
\mathbb{E}[ f(x_k) -f^*] \leq (1 - h\mu)^k (f(x_0) -f^*) + \frac{hL\sigma^2}{2\mu}
% \rightarrow \frac{hL\sigma^2}{2\mu}.
\end{equation}
for a constant learning rate, $h \leq \frac{1}{L}$.  In particular, with $h$ fixed, the function values converge exponentially, with rate $1 - h\mu$, to within $\frac{hL\sigma^2}{2\mu}$ of the optimal value. In Proposition \ref{prop:convergence neighborhood constant learning rate} we establish an accelerated version of~\eqref{eq: bottou inequality}: for $h \leq \frac{1}{\sqrt{L}}$, 
\begin{equation}
\label{eq: accelerated bottou inequality}
\mathbb{E}[ f(x_k) -f^*] \leq (1 - h\sqrt{\mu})^k E_0^{SC} + \frac{h\sigma^2}{2\sqrt{\mu}},
\end{equation}
where $E_0^{SC}$ is the initial value of a Lyapunov function. 
The inequality \eqref{eq: accelerated bottou inequality} shows that the exponential convergence rate of the previous results is accelerated, in the sense that the rate is now $1 - h\sqrt{\mu}$.   In addition, the neighborhood reached in \eqref{eq: accelerated bottou inequality} is smaller than the one reached in \eqref{eq: bottou inequality}. Other papers have studied accelerated versions of \eqref{eq: bottou inequality} using different methods, see for example \cite{Aybat2019,rabbat2020}. 
%Recently, this estimate has been improved using Nesterov's method with stochastic gradient \cite{Aybat2019,rabbat2020}. In their work, they show the usual accelerated rate and improve the constant in front of the variance. 
%Note that recently in \cite{Aybat2019}, the authors performed a similar Lyapunov analysis to obtain an accelerated version of \eqref{eq: bottou inequality} where $\mathbb{E}[f(x_k)]$ converges exponentially fast to a neighborhood of the minimum. In proposition \ref{prop:convergence neighborhood constant learning rate}, we recover this result. In addition, we show that if the initial Lyapunov function is smaller that a critical value, we obtain the accelerated convergence in expectation for the last iterate.

Both \eqref{eq: accelerated bottou inequality} and \eqref{eq: bottou inequality}, show that the convergence is improve by sending either the learning rate, $h$, or the variance, $\sigma^2$ to zero.  Variance reduction algorithms such as Stochastic Variance Reduction Gradient (SVRG) \cite{SVRG_2013}, Stochastic Average Gradient (SAG) \cite{SAG_2017} and SAGA \cite{SAGA_2014} aim at reducing the variance.  These methods consist in defining at each step a stochastic gradient, $\widehat{g}_k$, such that its variance converges to zero. However, in many modern applications, variance reduction is not effective~\cite{Defazio_Bottou_2019}.


\subsection{Improved convergence rate for the last iterate of SGD}
In this work, we focus on convergence rates for the last iterate of SGD, using a decreasing learning rate.  A typical learning rate schedule for SGD takes the form
\[
h_k = \frac 1 {\mu(k + k_0)}
\]
in the $\mu$-strongly convex case. Taking $k_0 = C_f$, ensures $	\alpha_k \leq \alpha_0 = 1 /L$, required for stability. 
%\begin{equation}
%	\label{alpha_cond}
%	\alpha_k \leq \alpha_0 = \frac 1 L.
%\end{equation}


Convergence results for averages of previous iterates are available in~\cite{Polyak_average_1992, Rakhkin2012, lacoste2012simpler, shamir2013stochastic}, for instance.  In \cite{AWBR_2009}, the authors proved that the optimal bound for the last iterate are $\mathcal{O}\left({1}/{\sqrt{k}} \right)$ (convex case) and $\mathcal{O}\left({1}/{k} \right)$ (strongly convex case).   Because the convergence rates are slow for SGD, improving the rate constant can make a difference: for the $1/k$ rate improving the constant by a factor of ten means the same error bound is achieved in one tenth the number of iterations.  In the rate constants which follow, $G^2$, is a bound for $\mathbb{E}[ \widehat g^2 ]$. 

 In the strongly convex case, we obtain the optimal $\mathcal{O}(1/k)$ rate for the last iterate, but improve the rate constant, be removing the dependance of the rate on the $L$-smoothness bound of the gradient.  (The constant, $L$, appears in the algorithm, to initialize the  learning rate, but not in the convergence rate).  Previous results,  \cite{nemirovski2009robust, shamir2013stochastic, jain2018accelerating}, have a rate which depends on $G$. See Table~\ref{fig: rates in expectation str convex}.
 
 In the convex case, the optimal rate for the last iterate of SGD (see \cite{shamir2013stochastic}) is order $\log(k)/\sqrt{k}$, with a rate constant that depends on $G^2$.  \cite{JainNN19} remove the log factor, by assuming that the number of iterations is decided in advance.   We obtain the $\mathcal{O}(\log(k)/\sqrt{k})$ rate for the last iterate, but again with removing the factor $G$ and the dependence on the $L$-smoothness.  See Table~\ref{fig: rates in expectation convex}. 	
 	
\begin{table*}[h!]
\caption{Convergence rate of $\mathbb{E}[f(x_k) -f^*]$ for a convex, $L$-smooth function.  $G^2$ is a bound on $\mathbb{E}[\widehat{g}^2 ]$, and $\sigma^2$ is a bound on the variance of $ \widehat{g}- \nabla f$. $h_k$ is the learning rate, $E_0$ is the initial value of the Lyapunov function. Top: $\mu$-strongly convex case, $h_k = \mathcal O (1/k)$. Bottom: convex case,   $D$ is the diameter of the domain,  $c$ is a free parameter.}
\label{fig: rates in expectation convex}
\label{fig: rates in expectation str convex}
\begin{center}
\begin{tabular}{|c|c|c|c|} 
\hline
 \cite{nemirovski2009robust}& \cite{shamir2013stochastic} &   \cite{JainNN19}  &  Acc. SGD (Prop~\ref{prop: decrease expectation E_k str convex acc}) \\ 
\hline 
 $ \dfrac{2C_f G^2}{\mu k }$ & $ \dfrac{17 G^2(1+ \log(k))}{\mu k }$ & $ \dfrac{130 G^2}{\mu k }$ &  $ \dfrac{4\sigma^2}{\mu k + \frac{4\sigma^2}{E_0^{SC}}}$ \\
\hline
\end{tabular}
%
\vspace{.2cm}
%
\begin{tabular}{|c|c|c|c|} 
\hline
 &\cite{shamir2013stochastic}&   Acc. SGD (Prop~\ref{prop: decrease expectation E_k convex acc}) \\ 
\hline 
$h_k$ & $\dfrac{c^2}{\sqrt{k}}$  &  $\dfrac{c}{ (k+1)^{3/4}}$\\  
\hline
 Rate &$\left(\dfrac{D^2}{c^2} + c^2 G^2 \right)\dfrac{(2+ \log(k))}{ \sqrt{k} }$
 & 
$ \dfrac{ \frac{E_0^C}{16c^2} + c^2 \sigma^2(1 +\log(k))}{\sqrt{k}}$
 \\
\hline
\end{tabular}
\end{center}

\end{table*}
 
  
\subsection{Nesterov's methods and Stochastic Gradient Descent}
Nesterov's method \cite{nesterov1983method} for accelerated gradient descent  can be written as 
\begin{align}
\label{genericN1}\tag{AGD1}
	x_{k+1} &= y_k - \frac 1 L \nabla f(y_k)\\
\label{genericN2}\tag{AGD2}
	y_{k+1} &= x_{k+1} + \beta_k(x_{k+1}-x_k)
\end{align}
The optimal choice of parameters is given by 
\begin{equation}
	\label{AGD_SC_params}
	\tag{Coeff-SC}
%	\alpha = \frac 1 L,  \qquad
\beta = \beta_k = \frac{\sqrt{C_f} - 1}{\sqrt{C_f} + 1}.
\end{equation}
in the $\mu$-strongly convex case, and 
\begin{equation}
	\label{AGD_Convex_params}
		\tag{Coeff-C}
%	\alpha = \frac 1 L,  \qquad
\beta_k = \frac{k}{k+3}
\end{equation}
in the convex case.  The general formulation of Nesterov's method involves three variables: the special cases above arise when one of the variables has been eliminated. 

Taking $\beta = 0$ recovers standard gradient descent.  
Popular heuristic methods for accelerated SGD consist of using the iteration \eqref{genericN1}\eqref{genericN2}, replacing $1/L$ with $h_k$, a decreasing learning rate, for example~\cite{kingma2014adam}. \red{The practical speed up does is lacking rigorous justification.  Our result, which gives an improved convergence rate to a very similar algorithm, can be seen as justification for the observed results?}



The accelerated stochastic gradient descent methods \red{we introduce} can be written as generalizations of  \eqref{genericN1}-\eqref{genericN2}.  We show that that decreasing learning rate versions of the ODEs which lead to Nesterov's method result in systems of the form
\begin{align}
\label{genericASGD1}\tag{ASGD1}
	x_{k+1} &= y_k - \frac{\alpha_k}{L} \nabla f(y_k)\\
\label{genericASGD2}\tag{ASGD2}
	y_{k+1} &= x_{k+1} + \beta_k(x_{k+1}-x_k) + \gamma_k (y_k - x_k)
\end{align}
% \red{typo? should it be $\nabla f(y_k)/L$ above to generalize from the full gradient case?}
where $\alpha_k,\beta_k$, and $\gamma_k$ are parameters.  (Note the additional parameter $\gamma$ which does not appear in other methods).  For example, in the strongly convex case,  we obtain, in  Proposition~\ref{prop: generalization Nesterov SC}
\[
\alpha_k = \frac {\sqrt{C_f}}{ \sqrt{C_f} + k/2}, \qquad \beta_{k} = \frac{\sqrt{C_f} - 1}{\sqrt{C_f} + 1 + k/2 }, \qquad \gamma_k = \frac{k }{2\sqrt{C_f} +k + 3},
\]  
These coefficients reduce to~\eqref{AGD_SC_params} when $k=0$.  In the convex case, Proposition \ref{prop: generealization Nesterov C} leads to the following coefficients
\[
\alpha_k =\sqrt{L} h_k,
	\qquad
	\beta_k = \frac{h_{k+1}}{t_{k+1}}(t_k \sqrt{L} -1)  %\frac{w_{k+1}}{w_{k}}\left(1 - w_k \right)
		\qquad
	\gamma_k = \frac{t_k}{t_{k+1}} \frac{h_{k+1}}{h_k}(1 - \sqrt{L}h_k) %\frac{w_{k+1}}{w_{k}} \left( 1 - h_k\sqrt{L} \right),
\] 
where $h_k = \frac{c}{(k+1)^{3/4}}$ and $t_k = \sum_{i=0}^k h_i$.  
%\red{check this} 
which also generalizes the convex coefficients \eqref{AGD_Convex_params}, when $h_k = \frac{1}{\sqrt{L}}$ and $t_k = h_k(k+2)$.
%although this is not immediately obvious. 


\subsection{Outline of our approach}    
%One goal of the continuous time approach is to take advantage of the Lyapunov function to obtain convergence rates for differential equations, with the hope that an explicit discretization of the differential equation leads to an algorithm which also decreases the Lyapunov function. 
~
%\red{reconsider this subsection, what is needed here?}

SGD can be interpreted as a time discretization of the gradient descent ODE, $\dot x(t) = -\nabla f(x(t))$, with perturbed gradients i.e. $\nabla f +e$. It is well-known that solutions of the ODE decrease a rate-generating Lyapunov function. In the perturbed case, an error term will appear in the dissipation of the Lyapunov function. This error can be handle choosing a specific schedule for the time step/learning rate, \cite{bottou2016optimization,Oberman_Prazeres}. \red{ cite our AISTATS paper?}\\ 
In what follows, we study accelerated methods for stochastic gradient descent.
The analysis we perform comes from writing the accelerated algorithm using a three variable formulations.  We present a derivation of Nesterov's method as a coupling between two gradient descent evolutions, where one is faster. We extend this analysis to a system of ODEs for accelerated gradient descent, which also has an associated Lyapunov function. The Lyapunov analysis in the accelerated case is substantially more complex than in the gradient descent case.  

The key step is to obtain the following dissipation of a discret rate-generating Lyapunov function $E_k$ during one step %inequality on a rate-generating Lyapunov function. 
\begin{equation}\label{inequ_main}
E_{k+1}
 \leq (1-\sqrt{\mu}h_k) E_{k+1}  + h_k\beta_k.
\end{equation}
Here, $h_k$ is the learning rate and the term  $\beta_k$ depends on the error $e_k$ from \eqref{perturbed_gradient}, which reduces to zero in the full gradient case $e =  0$. 
When we take expectations in \eqref{inequ_main}, $\mathbb{E}[\beta_k]$ is proportional to  $h_k \sigma^2$, see Proposition \ref{thm:Acc GD SC} in the strongly convex case and Proposition \ref{prop: different gaps convex acc perturbed} in the convex case,
\[
\mathbb{E}[E_{k+1}]
 \leq (1-\sqrt{\mu}h_k) \mathbb{E}[E_{k}]  + A_k h_k^2 \sigma^2,
\]
where $A_k$ is a contant which may depends on $k$. Choosing a particular $h_k$ allows us to sum up the error terms and obtain the accelerated rate of convergence presented in Table~\ref{fig: rates in expectation str convex}.
%The inequality \eqref{inequ_main} can be seen as a generalization of the fundamental lemma in \cite{bottou2016optimization}, where the objective is replaced by a Lyapunov function. 

\cite{SLRB11} used a related approach, but they considered the case where the magnitude of the errors decrease quickly enough to obtain the rates in the deterministic case.  A continuous time version of the analysis from \cite{SLRB11} was performed in \cite{attouch2016fast}. 

\subsection{Other related work}
 Continuous time analysis also appears in \cite{flammarion2015averaging}, \cite{lessard2016analysis}, and  \cite{NIPS2015_5843}, among many other recent works. The Lyapunov approach to proving convergence rates appears widely in optimization, for example, see \cite{beck2009fast} for FISTA. 

Convergence rates for averaged SGD are available in a wide setting, (\cite{bottou2016optimization}, \cite{lacoste2012simpler,Rakhkin2012,qian2019sgd}). In the non-asymptotic regime, the last iterate of SGD is often preferred in current applications.  The optimal convergence rate for SGD  is $O(1/k)$ in the smooth, strongly convex case, and $O(1/\sqrt{k})$ in the convex, nonsmooth case~(\cite{nemirovski2009robust}, \cite{bubeck2014optimization}).

When SGD is combined with momentum  (\cite{polyak1964some,nesterov2013introductory}) empirical performance is improved, but this improvement is not always theoretically established~(\cite{kidambi2018insufficiency}).  
 Accelerated versions of  stochastic gradient descent algorithms are comparatively more recent: they appear in \cite{lin2015universal} as well as in \cite{frostig2015regularizing} and \cite{jain2018accelerating}.  A direct acceleration method with a connection to Nesterov's method can be found in~\cite{allen2017katyusha}. \\


\paragraph{\textbf{Organization:}} 
We organize the paper as follows. In Section \ref{section: derivation Nest SC}, we derive our Accelerated Stochastic Gradient Descent and in Section \ref{section: accelerated str convex}, we study the rate convergence  of the last iterate of this scheme based on a Lyapunov analysis, in the strongly convex case. Then, in Sections \ref{section: accelerated convex} and \ref{section: derivation Nest C}, we study the convex case, first deriving a new algorithm and, then, studying the dissipation of a Lyapunov function. Finally, in the last Section \ref{section: simulations}, we present numerical simulations.


% Section \ref{section: abstract Liap} is devoted to the presentation of an abstract Lyapunov analysis. We 
%apply this analysis in the full gradient, and the stochastic gradient case.  In Section \ref{section:application} we apply the abstract analysis to the gradient descent ODE, in the case of convex and strongly convex functions.  
%
%Finally, in Sections \ref{section: accelerated convex} and \ref{section: accelerated str convex} we study the accelerated ODEs, and the related Lyapunov functions in the convex and strongly convex cases, respectively.   In the convex case we show that the discretization of \eqref{NODE} below  leads to Nesterov's method with a constant learning rate.  However setting the learning rate to  $h_k = O(k^{-3/4})$ in~\eqref{FEg},  (which is different from the usual order $k^{-1/2}$ rate) leads to an accelerated stochastic gradient descent algorithm. 
%In the strongly convex case, we begin with the ODE, \eqref{NODESC}, which is discretized with a learning rate $h_k$ to result in \eqref{FE-SC}.  In the full gradient case, setting the constant learning rate $h_k = 1/\sqrt L$ leads to Nesterov's method.  In the stochastic gradient case, setting $h_k = O(1/k)$ as described in Proposition~\ref{prop: decrease expectation E_k str convex acc},  leads to an accelerated SGD algorithm.\\  





